Fast View Synthesis of Casual Videos with Soup-of-Planes

Novel view synthesis from an in-the-wild video is difficult due to challenges like scene dynamics and lack of parallax. While existing methods have shown promising results with implicit neural radiance fields, they are slow to train and render. This paper revisits explicit video representations to synthesize high-quality novel views from a monocular video efficiently. We treat static and dynamic video content separately. Specifically, we build a global static scene model using an extended plane-based scene representation to synthesize temporally coherent novel video. Our plane-based scene representation is augmented with spherical harmonics and displacement maps to capture view-dependent effects and model non-planar complex surface geometry. We opt to represent the dynamic content as per-frame point clouds for efficiency. While such representations are inconsistency-prone, minor temporal inconsistencies are perceptually masked due to motion. We develop a method to quickly estimate such a hybrid video representation and render novel views in real time. Our experiments show that our method can render high-quality novel views from an in-the-wild video with comparable quality to state-of-the-art methods while being 100x faster in training and enabling real-time rendering.

==> figures/fig5.5_nvidia_long.tex <==
\begin{figure}
\vspace{-2mm}
\centering
\includegraphics[trim={8.4cm 5.7cm 8.5cm 5.9cm},clip,width=\linewidth]{figures/pdfs/nvidia_long.pdf}
\vspace{0mm}
\vspace{-7.8mm}
\caption{\textbf{Quantitative and speed comparison using the NVIDIA-long protocol~\cite{dynibar}.} Although DynIBaR~\cite{dynibar} gets the best quality overall, it is time-consuming for training and rendering. In contrast, with the fastest training and rendering speed, the rendering quality of our method is the second-best in the LPIPS metric, and comparable with DynNeRF~\cite{gao2021dynerf} and NSFF~\cite{nsff} and better than FlowIBR~\cite{busching2023flowibr} in the 
PSNR metric.
\vspace{-0.13in}}
\label{fig:nvidia_long_quantitative}
\end{figure}

==> figures/fig6_visual_comp_nvidia_long.tex <==
\begin{figure}
    \centering
    \frame{\includegraphics[width=0.19\linewidth]{figures/fig6_assets/balloon1/crop_gt.png}}
    \frame{\includegraphics[width=0.19\linewidth]{figures/fig6_assets/balloon1/crop_ours.png}}
    \frame{\includegraphics[width=0.19\linewidth]{figures/fig6_assets/balloon1/crop_nsff.png}}
    \frame{\includegraphics[width=0.19\linewidth]{figures/fig6_assets/balloon1/crop_dvs.png}}
    \frame{\includegraphics[width=0.19\linewidth]{figures/fig6_assets/balloon1/crop_dynibar.png}}
    \\
    \vspace{0.5mm}
    \frame{\includegraphics[width=0.19\linewidth]{figures/fig6_assets/balloon2/crop_gt.png}}
    \frame{\includegraphics[width=0.19\linewidth]{figures/fig6_assets/balloon2/crop_ours.png}}
    \frame{\includegraphics[width=0.19\linewidth]{figures/fig6_assets/balloon2/crop_nsff.png}}
    \frame{\includegraphics[width=0.19\linewidth]{figures/fig6_assets/balloon2/crop_dvs.png}}
    \frame{\includegraphics[width=0.19\linewidth]{figures/fig6_assets/balloon2/crop_dynibar.png}}
    \\
    \vspace{-1.4mm}
    \begin{subfigure}{0.19\linewidth}\centering\scriptsize
        Groundtruth
    \end{subfigure}
    \begin{subfigure}{0.19\linewidth}\centering\scriptsize
        Ours
    \end{subfigure}
    \begin{subfigure}{0.19\linewidth}\centering\scriptsize
        NSFF~\cite{nsff}
    \end{subfigure}
    \begin{subfigure}{0.19\linewidth}\centering\scriptsize
        DynNeRF~\cite{gao2021dynerf}
    \end{subfigure}
    \begin{subfigure}{0.19\linewidth}\centering\scriptsize
        DynIBaR~\cite{dynibar}
    \end{subfigure}
\vspace{-2.5mm}
\caption{
\textbf{Visual comparison on NVIDIA-long protocol~\cite{dynibar}.} While the dynamic content in our results slightly misaligns with the ground truth due to the ill-posed dynamic depth estimation problem, our results are sharp with richer details than~\cite{nsff,gao2021dynerf}.}%NSFF and DynNeRF.}
\vspace{-6mm}
\label{fig:nvidia_long_visual}
\end{figure}


==> figures/fig_reb_3dgs.tex <==
\begin{figure}[H]
\centering
\includegraphics[width=\linewidth, clip, trim={0 13cm 4.5cm 0}]{figures/eccv_rebuttal/rebuttal_3dgs.pdf}
% \vspace{-9.5mm}
% \caption{Regularized 3DGS still fails in the weak-parallax scene.}
% \vspace{-3.8mm}
% \label{fig:reb-3dgs}
\end{figure}

==> figures/fig_reb_yang_4dgs.tex <==
\begin{figure}[H]
\centering
\includegraphics[width=\linewidth, clip, trim={0 13cm 4.5cm 0}]{figures/eccv_rebuttal/rebuttal_4dgs.pdf}
% \vspace{-9mm}
% \caption{Comparison to Yang~\etal~[83], depth shown in the right. }
% \vspace{-4.8mm}
% \label{fig:reb-4dgs}
\end{figure}

==> figures/fig_supp_3dgs_ambiguity.tex <==
\begin{wrapfigure}{r}{0.25\textwidth}
\centering
\vspace{-0.6cm}\includegraphics[trim={0.1cm 4.4cm 27cm 0.2cm},clip,keepaspectratio,scale=0.3]{figures/pdfs/supp_3dgs_ambiguity.pdf}
% \vspace{-8mm}
\caption{{\textbf{Ambiguities of 3DGS in weak-parallax scenes.}}
}
\vspace{-7mm}
\label{fig:supp_plane_visualization}
\end{wrapfigure}

==> figures/fig_supp_model_size.tex <==
\begin{figure}
\includegraphics[trim={0.5cm 14cm 14cm 0.1cm},clip,width=\linewidth]{figures/pdfs/supp_model_size.pdf}
\vspace{-4mm}
\caption{{\textbf{Model size comparison.}}
We present the trade-off between the visual quality and model size, focusing primarily on the view-dependent appearance texture maps $\C^{0..\ell_{\max}^{\C}}$.
However, it's important to note that in the first and second columns, our proposed view-dependent displacement maps $\Delta^{0..\ell_{\max}^{\Delta}}$ are capable of retaining more complex scene details even without relying on view-dependent appearance, and this comes at a mere additional 5MB in size.
}
\vspace{-7mm}
\label{fig:supp_model_size}
\end{figure}

==> figures/fig_supp_nvidia_part1.tex <==
\begin{figure*}[ht]
    \centering
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Balloon1/gt.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Balloon1/Ours.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Balloon1/HyperNeRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Balloon1/NSFF.png}}
    \\
    \vspace{-1mm}
    \begin{subfigure}{0.24\linewidth}\centering\small
        Ground Truth
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        Ours
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        HyperNeRF~\cite{gao2021dynerf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        NSFF~\cite{nsff}
    \end{subfigure}
    \\
    \vspace{1.5mm}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Balloon1/DynamicNeRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Balloon1/RoDynRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Balloon1/MonoNeRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Balloon1/4DGS.png}}
    \\
    \vspace{-1mm}
    \begin{subfigure}{0.24\linewidth}\centering\small
        DynNeRF~\cite{gao2021dynerf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        RoDynRF~\cite{robustdynrf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        MonoNeRF~\cite{tian2023mononerf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        4D-GS~\cite{wu4dgaussians}
    \end{subfigure}
    \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \vspace{4mm}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Playground/gt.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Playground/Ours.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Playground/HyperNeRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Playground/NSFF.png}}
    \\
    \vspace{-1mm}
    \begin{subfigure}{0.24\linewidth}\centering\small
        Groundt Truth
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        Ours
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        HyperNeRF~\cite{gao2021dynerf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        NSFF~\cite{nsff}
    \end{subfigure}
    \\
    \vspace{1.5mm}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Playground/DynamicNeRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Playground/RoDynRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Playground/MonoNeRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Playground/4DGS.png}}
    \\
    \vspace{-1mm}
    \begin{subfigure}{0.24\linewidth}\centering\small
        DynNeRF~\cite{gao2021dynerf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        RoDynRF~\cite{robustdynrf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        MonoNeRF~\cite{tian2023mononerf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        4D-GS~\cite{wu4dgaussians}
    \end{subfigure}
    \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \vspace{4mm}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Truck/gt.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Truck/Ours.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Truck/HyperNeRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Truck/NSFF.png}}
    \\
    \vspace{-1mm}
    \begin{subfigure}{0.24\linewidth}\centering\small
        Ground Truth
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        Ours
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        HyperNeRF~\cite{gao2021dynerf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        NSFF~\cite{nsff}
    \end{subfigure}
    \\
    \vspace{1.5mm}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Truck/DynamicNeRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Truck/RoDynRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Truck/MonoNeRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Truck/4DGS.png}}
    \\
    \vspace{-1mm}
    \begin{subfigure}{0.24\linewidth}\centering\small
        DynNeRF~\cite{gao2021dynerf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        RoDynRF~\cite{robustdynrf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        MonoNeRF~\cite{tian2023mononerf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        4D-GS~\cite{wu4dgaussians}
    \end{subfigure}
    \\
    
\vspace{-3mm}
\caption{
\textbf{Visual comparison on the NVIDIA dataset.} 
\vspace{-0.1in}
}
\label{fig:supp_nvidia_visual1}
\end{figure*}

==> figures/fig_supp_nvidia_part2.tex <==
\begin{figure*}[ht]
    \centering
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Skating/gt.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Skating/Ours.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Skating/HyperNeRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Skating/NSFF.png}}
    \\
    \vspace{-1mm}
    \begin{subfigure}{0.24\linewidth}\centering\small
        Ground Truth
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        Ours
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        HyperNeRF~\cite{gao2021dynerf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        NSFF~\cite{nsff}
    \end{subfigure}
    \\
    \vspace{1.5mm}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Skating/DynamicNeRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Skating/RoDynRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Skating/MonoNeRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Skating/4DGS.png}}
    \\
    \vspace{-1mm}
    \begin{subfigure}{0.24\linewidth}\centering\small
        DynNeRF~\cite{gao2021dynerf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        RoDynRF~\cite{robustdynrf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        MonoNeRF~\cite{tian2023mononerf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        4D-GS~\cite{wu4dgaussians}
    \end{subfigure}
    \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \vspace{4mm}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Umbrella/gt.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Umbrella/Ours.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Umbrella/HyperNeRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Umbrella/NSFF.png}}
    \\
    \vspace{-1mm}
    \begin{subfigure}{0.24\linewidth}\centering\small
        Ground Truth
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        Ours
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        HyperNeRF~\cite{gao2021dynerf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        NSFF~\cite{nsff}
    \end{subfigure}
    \\
    \vspace{1.5mm}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Umbrella/DynamicNeRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Umbrella/RoDynRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Umbrella/MonoNeRF.png}}
    \frame{\includegraphics[width=0.24\linewidth]{figures/supp_fig_nvidia_assets/Umbrella/4DGS.png}}
    \\
    \vspace{-1mm}
    \begin{subfigure}{0.24\linewidth}\centering\small
        DynNeRF~\cite{gao2021dynerf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        RoDynRF~\cite{robustdynrf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        MonoNeRF~\cite{tian2023mononerf}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}\centering\small
        4D-GS~\cite{wu4dgaussians}
    \end{subfigure}
    \\
    
\vspace{-3mm}
\caption{
\textbf{Visual comparison on the NVIDIA dataset.} 
\vspace{-0.1in}
}
\label{fig:supp_nvidia_visual2}
\end{figure*}

==> figures/fig_supp_plane_visualization.tex <==
\begin{figure}
\includegraphics[trim={0.155cm 14cm 10.45cm 0.94cm},clip,width=\linewidth]{figures/pdfs/plane_visualization.pdf}
\vspace{-8mm}
\caption{{\textbf{Visualizations of soup-of-planes.}}
We fit a set of 3D-oriented planes onto the static-scene point cloud in the plane initialization step.
}
\vspace{-7mm}
\label{fig:supp_plane_visualization}
\end{figure}

==> figures/fig_supp_view_dependent_displacement.tex <==
\begin{figure}
\centering
\includegraphics[trim={0.1cm 11cm 19cm 0.1cm},clip,width=0.7\linewidth]{figures/pdfs/supp_view_independent_displacement.pdf}
\vspace{-4mm}
\caption{{\textbf{Efficacy of view-dependent texture displacement.}}
We compare the proposed view-dependent texture displacement with two baseline approaches. In the middle column, we employ a view-independent displacement by setting $\ell_{\max}^{\Delta}$ to 0. While view-independent displacement can help redistribute texture space to preserve high-frequency details more effectively than without texture displacement (left column), it remains inadequate in accurately modeling the diverse ray-plane intersections of a complex surface. In contrast, the proposed view-dependent texture displacement handles the complex geometry, resulting in superior rendering quality (right column).
}
% \vspace{-7mm}
\label{fig:supp_view_dependent_displace}
\end{figure}

==> tables/supp_tb_render_time.tex <==
\begin{table}
\caption{\textbf{Rendering runtime breakdown.} The experiment is conducted on a single A100 GPU with an 80-frame input video of 860\texttimes 480 resolution. The proposed method achieves real-time rendering at 27 FPS.}
\scriptsize
\centering
\begin{tabular}{lL{3.8cm}r}
\hline
\multicolumn{2}{l}{Rendering step} & \multicolumn{1}{c}{Runtime (ms)} \\ \hline
\multirow{4}{*}{Static} & Obtain view-dep. texture & 1.99 \\
 & Plane warping & 12.42 \\
 & Pixelwise depth sorting & 0.12 \\
 & Plane composition & 0.27 \\ \hline
\multirow{2}{*}{Dynamic} & Neighboring blending & 21.28 \\
 & Forward splatting & 1.35 \\ \hline
\multicolumn{2}{l}{Static-dynamic composition} & 0.09 \\ \hline
Total &  & 37.52 \\ \hline
\end{tabular}


\label{tbl:supp_rendering_runtime_breakdown}
\end{table}

==> tables/supp_tb_train_time.tex <==
\begin{table}
\caption{\textbf{Training runtime breakdown.} We run the experiment on a single A100 GPU with an 80-frame input video of 860x480 resolution. Our method is efficient to supervise and trains on casual videos within 15 minutes.}
\scriptsize
\centering
\begin{tabular}{lL{3.2cm}r}
\hline
\multicolumn{2}{l}{Training step} & \multicolumn{1}{l}{Runtime (sec)} \\ \hline
\multirow{3}{*}{Initialization} & Plane geometry fitting & 22.2 \\
 & Plane texture & 1.2 \\
 & Dynamic model & 2.4 \\ \hline
\multicolumn{2}{l}{Scene representation optimization} & 782.0 \\ \hline
\multicolumn{2}{l}{Total} & 807.8 \\ \hline
\end{tabular}

\label{tbl:supp_training_runtime_breakdown}
\end{table}

==> tables/tb1_nvidia_quantitative.tex <==

\begin{table}

\caption{\textbf{Quantitative comparison on the NVIDIA dataset~\cite{yoon2020nvidia}.}
We highlight the \textbf{best} and \ul{second best} for each column.
We adopt the numbers reported by RoDynRF~\cite{robustdynrf}.
Yoon~\etal~\cite{yoon2020nvidia}'s results only contain the middle 10 frames provided by RoDynRF~\cite{robustdynrf}.
%For the per-scene optimization results of MonoNeRF~\cite{tian2023mononerf}, we provide both the reported numbers in their paper and the reproduced results$\dagger$ by their official codes. 
The per-scene optimization results of MonoNeRF~\cite{tian2023mononerf} are adopted from their paper.
The results of 4D-GS~\cite{wu4dgaussians} are produced by their official codes. Our method achieves the second-best in the LPIPS metric. We highlight the best in red and the second best in yellow.
}
\vspace{-2mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c@{\extracolsep{6pt}}c|c@{\extracolsep{6pt}}c|c@{\extracolsep{6pt}}c|c@{\extracolsep{6pt}}c|c@{\extracolsep{6pt}}c|c@{\extracolsep{6pt}}c|c@{\extracolsep{6pt}}c|c@{\extracolsep{6pt}}c}
\toprule
\multicolumn{1}{c|}{PSNR \textuparrow / LPIPS \textdownarrow} & \multicolumn{2}{c|}{Jumping} & \multicolumn{2}{c|}{Skating} & \multicolumn{2}{c|}{Truck} & \multicolumn{2}{c|}{Umbrella} & \multicolumn{2}{c|}{Balloon1} & \multicolumn{2}{c|}{Balloon2} & \multicolumn{2}{c|}{Playground} & \multicolumn{2}{c}{Average} \\ \midrule
Yoon~\etal~\cite{yoon2020nvidia} & 20.15 & 0.148 & 21.75 & 0.135 & 21.53 & 0.099 & 20.35 & 0.179 & 18.74 & 0.179 & 19.88 & 0.139 & 15.08 & 0.184 & 19.64 & 0.152 \\
Ours (10 frames) & 22.60 & 0.107 & 29.23 & 0.049 & 22.68 & 0.079 & 22.58 & 0.109 & 22.98 & 0.088 & 23.51 & 0.088 & 21.42 & 0.082 & 23.57 & 0.086 \\ \midrule
D-NeRF~\cite{dnerf2021} & 22.36 & 0.193 & 22.48 & 0.323 & 24.10 & 0.145 & 21.47 & 0.264 & 19.06 & 0.259 & 20.76 & 0.277 & 20.18 & 0.164 & 21.48 & 0.232 \\
NR-NeRF~\cite{tretschk2021nrnerf} & 20.09 & 0.287 & 23.95 & 0.227 & 19.33 & 0.446 & 19.63 & 0.421 & 17.39 & 0.348 & 22.41 & 0.213 & 15.06 & 0.317 & 19.69 & 0.323 \\
TiNeuVox~\cite{tineuvox} & 20.81 & 0.247 & 23.32 & 0.152 & 23.86 & 0.173 & 20.00 & 0.355 & 17.30 & 0.353 & 19.06 & 0.279 & 13.84 & 0.437 & 19.74 & 0.285 \\
HyperNeRF~\cite{hypernerf} & 18.34 & 0.302 & 21.97 & 0.183 & 20.61 & 0.205 & 18.59 & 0.443 & 13.96 & 0.530 & 16.57 & 0.411 & 13.17 & 0.495 & 17.60 & 0.367 \\
DynNeRF~\cite{gao2021dynerf} & \cellcolor[HTML]{FFFFC7}24.68 & \cellcolor[HTML]{FFFFC7}0.090 & \cellcolor[HTML]{FFCCC9}32.66 & \cellcolor[HTML]{FFCCC9}0.035 & \cellcolor[HTML]{FFFFC7}28.56 & \cellcolor[HTML]{FFFFC7}0.082 & 23.26 & 0.137 & 22.36 & 0.104 & \cellcolor[HTML]{FFFFC7}27.06 & \cellcolor[HTML]{FFCCC9}0.049 & \cellcolor[HTML]{FFFFC7}24.15 & 0.080 & \cellcolor[HTML]{FFCCC9}26.10 & 0.082 \\
NSFF~\cite{nsff} & 24.65 & 0.151 & 29.29 & 0.129 & 25.96 & 0.167 & 22.97 & 0.295 & 21.96 & 0.215 & 24.27 & 0.222 & 21.22 & 0.212 & 24.33 & 0.199 \\
RoDynRF~\cite{robustdynrf} & \cellcolor[HTML]{FFCCC9}25.66 & \cellcolor[HTML]{FFCCC9}0.071 & 28.48 & \cellcolor[HTML]{FFFFC7}0.040 & \cellcolor[HTML]{FFCCC9}29.13 & \cellcolor[HTML]{FFCCC9}0.063 & \cellcolor[HTML]{FFCCC9}24.26 & \cellcolor[HTML]{FFCCC9}0.089 & \cellcolor[HTML]{FFFFC7}22.37 & \cellcolor[HTML]{FFFFC7}0.103 & 26.19 & 0.054 & \cellcolor[HTML]{FFCCC9}24.96 & \cellcolor[HTML]{FFCCC9}0.048 & \cellcolor[HTML]{FFFFC7}25.89 & \cellcolor[HTML]{FFCCC9}0.065 \\
MonoNeRF~\cite{tian2023mononerf} & 24.26 & 0.091 & \cellcolor[HTML]{FFFFC7}32.06 & 0.044 & 27.56 & 0.115 & \cellcolor[HTML]{FFFFC7}23.62 & 0.180 & 21.89 & 0.219 & \cellcolor[HTML]{FFCCC9}27.36 & \cellcolor[HTML]{FFFFC7}0.052 & 22.61 & 0.130 & 25.62 & 0.106 \\
4D-GS~\cite{wu4dgaussians} & 21.03 & 0.269 & 24.84 & 0.174 & 23.02 & 0.175 & 21.83 & 0.213 & 21.32 & 0.185 & 18.81 & 0.178 & 18.40 & 0.196 & 21.45 & 0.199 \\
Ours & 23.45 & 0.100 & 29.98 & 0.045 & 25.22 & 0.090 & 23.24 & \cellcolor[HTML]{FFFFC7}0.096 & \cellcolor[HTML]{FFCCC9}23.75 & \cellcolor[HTML]{FFCCC9}0.079 & 24.15 & 0.081 & 22.19 & \cellcolor[HTML]{FFFFC7}0.074 & 24.57 & \cellcolor[HTML]{FFFFC7}0.081 \\ \bottomrule
\end{tabular}
}
\vspace{-4.5mm}
\label{tbl:nvidia_12}
\end{table}
% \end{landscape}

==> tables/tb2_nvidia_long_quantitative.tex <==
\makeatletter
\newcommand*\tabletwosize{%
  \@setfontsize\tabletwosize{7.6}{10.0}%
}

\begin{table}
\tabletwosize
\begin{tabular}{L{1.7cm}R{0.67cm}R{0.64cm}R{0.64cm}R{0.64cm}R{0.64cm}R{0.64cm}}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{Methods}} & \multicolumn{3}{c}{Full} & \multicolumn{3}{c}{Dynamic-only} \\
\multicolumn{1}{c}{} & \scriptsize{SSIM\textuparrow} & \scriptsize{PSNR\textuparrow} & \scriptsize{LPIPS\textdownarrow} & \scriptsize{SSIM\textuparrow} & \scriptsize{PSNR\textuparrow} & \scriptsize{LPIPS\textdownarrow} \\ \hline
Nerfies*~\cite{nerfies} & 0.609 & 20.64 & 0.204 & 0.455 & 17.35 & 0.258 \\
HyperNeRF*~\cite{hypernerf} & 0.654 & 20.90 & 0.182 & 0.446 & 17.56 & 0.242 \\
DynNeRF*~\cite{gao2021dynerf} & 0.921 & 27.44 & 0.070 & 0.778 & 22.63 & 0.144 \\
NSFF*~\cite{nsff} & \ul{0.927} & \ul{28.90} & 0.062 & \ul{0.783} & \ul{23.08} & 0.159 \\
DynIBaR*~\cite{dynibar} & \textbf{0.957} & \textbf{30.86} & \textbf{0.027} & \textbf{0.824} & \textbf{24.24} & \textbf{0.062} \\
FlowIBR$\dagger$~\cite{busching2023flowibr} & 0.692 & 26.88 & 0.096 & 0.680 & 21.12 & 0.201 \\
Ours & 0.886 & 26.96 & \ul{0.050} & 0.623 & 19.87 & \ul{0.113} \\ \hline
\end{tabular}
\caption{\textbf{Quantitative comparison on Nvidia-Long Protocol~\cite{dynibar}.}
The best and second best are highlighted as \textbf{bold} and \ul{underline.} The numbers indicated by * are adopted from DynIBaR~\cite{dynibar}, and $\dagger$ from FlowIBR~\cite{busching2023flowibr}. Although DynIBaR achieves the best scores, it requires 40 hours for per scene optimization. By contrast, the proposed method performs the second best LPIPS scores within 15 minutes.
}
\label{tbl:nvidia_long}
\end{table}

==> tables/tb_supp_scene_flow.tex <==
\makeatletter
\newcommand*\tablesupponesize{%
  \@setfontsize\tablesupponesize{6}{10.0}%
}
\makeatother

\begin{table*}[t]
\caption{\textbf{Ablation on scene flow regularization.}
Although the scene flow regularization $\L_{sf}$ can improve the scores of three examples by better aligning with the ground-truths, the quality of the other four examples degrades due to the over-smoothed dynamic depths caused by the regularization. Additionally, the scene flow regularization doubles the training time. Hence, we disable the scene flow regularization by default. Without the regularization, our method can still render visually plausible dynamics in spite of some slight misalignments with the ground truth. We encourage our readers to view our %\href{run:index.html}{demo webpage} 
demo webpage to see the video synthesis results of casual videos.
}
\tablesupponesize
\resizebox{\textwidth}{!}{\begin{tabular}{L{1.8cm}|c|ccccccc|c}
\hline
\multicolumn{1}{c|}{PSNR \textuparrow / LPIPS \textdownarrow} & Train time & Jumping & Skating & Truck & Umbrella & Balloon1 & Balloon2 & Playground & Average \\ \hline
%Yoon~\etal~\cite{yoon2020nvidia} & 20.15 / 0.148 & 21.75 / 0.135 & 21.53 / 0.099 & 20.35 / 0.179 & 18.74 / 0.179 & 19.88 / 0.139 & 15.08 / 0.184 & 19.64 / 0.152 \\
%Ours (10 frames) & 22.60 / 0.107 & 29.23 / 0.049 & 22.68 / 0.079 & 22.58 / 0.109 & 22.98 / 0.088 & 23.56 / 0.087 & 21.39 / 0.083 & 23.57 / 0.086 \\ \hline
%D-NeRF*~\cite{dnerf2021} & \multicolumn{1}{l}{22.36 / 0.193} & \multicolumn{1}{l}{22.48 / 0.323} & \multicolumn{1}{l}{24.10 / 0.145} & \multicolumn{1}{l}{21.47 / 0.264} & \multicolumn{1}{l}{19.06 / 0.259} & \multicolumn{1}{l}{20.76 / 0.277} & \multicolumn{1}{l|}{20.18 / 0.164} & \multicolumn{1}{l}{21.48 / 0.232} \\
%NR-NeRF*~\cite{tretschk2021nrnerf} & \multicolumn{1}{l}{20.09 / 0.287} & \multicolumn{1}{l}{23.95 / 0.227} & \multicolumn{1}{l}{19.33 / 0.446} & \multicolumn{1}{l}{19.63 / 0.421} & \multicolumn{1}{l}{17.39 / 0.348} & \multicolumn{1}{l}{22.41 / 0.213} & \multicolumn{1}{l|}{15.06 / 0.317} & \multicolumn{1}{l}{19.69 / 0.323} \\
%TiNeuVox*~\cite{tineuvox} & \multicolumn{1}{l}{20.81 / 0.247} & \multicolumn{1}{l}{23.32 / 0.152} & \multicolumn{1}{l}{23.86 / 0.173} & \multicolumn{1}{l}{20.00 / 0.355} & \multicolumn{1}{l}{17.30 / 0.353} & \multicolumn{1}{l}{19.06 / 0.279} & \multicolumn{1}{l|}{13.84 / 0.437} & \multicolumn{1}{l}{19.74 / 0.285} \\
%HyperNeRF*~\cite{hypernerf} & \multicolumn{1}{l}{18.34 / 0.302} & \multicolumn{1}{l}{21.97 / 0.183} & \multicolumn{1}{l}{20.61 / 0.205} & \multicolumn{1}{l}{18.59 / 0.443} & \multicolumn{1}{l}{13.96 / 0.530} & \multicolumn{1}{l}{16.57 / 0.411} & \multicolumn{1}{l|}{13.17 / 0.495} & \multicolumn{1}{l}{17.60 / 0.367} \\
%NSFF*~\cite{nsff} & \multicolumn{1}{l}{24.65 / 0.151} & \multicolumn{1}{l}{29.29 / 0.129} & \multicolumn{1}{l}{25.96 / 0.167} & \multicolumn{1}{l}{22.97 / 0.295} & \multicolumn{1}{l}{21.96 / 0.215} & \multicolumn{1}{l}{24.27 / 0.222} & \multicolumn{1}{l|}{21.22 / 0.212} & \multicolumn{1}{l}{24.33 / 0.199} \\
%DynNeRF*~\cite{gao2021dynerf} & \multicolumn{1}{l}{{24.68} / {0.090}} & \multicolumn{1}{l}{{32.66} / {0.035}} & \multicolumn{1}{l}{{28.56} / {0.082}} & \multicolumn{1}{l}{23.26 / 0.137} & \multicolumn{1}{l}{22.36 / 0.104} & \multicolumn{1}{l}{{27.06} / {0.049}} & \multicolumn{1}{l|}{{24.15} / 0.080} & \multicolumn{1}{l}{{26.10} / 0.082} \\
%RoDynRF*~\cite{robustdynrf} & {25.66} / {0.071} & 28.68 / {0.040} & {29.13} / {0.063} & {24.26} / {0.089} & {22.37} / {0.103} & 26.19 / 0.054 & {24.96} / {0.048} & {25.89} / {0.065} \\
%MonoNeRF~\cite{tian2023mononerf} & 24.26 / 0.091 & {32.06} / 0.044 & 27.56 / 0.115 & {23.62} / 0.180 & 21.89 / 0.129 & {27.36} / {0.052} & 22.61 / 0.130 & 25.62 / 0.106 \\
%MonoNeRF$\dagger$~\cite{tian2023mononerf} & 23.47 / 0.091 & 27.02 / 0.057 & 27.90 / 0.103 & 22.61 / 0.179 & 21.74 / 0.129 & \ul{27.09} / 0.054 & 22.04 / 0.111 & 24.55 / 0.103 \\
%4D-GS~\cite{wu4dgaussians} & 21.93 / 0.269 & 24.84 / 0.174 & 23.02 / 0.175 & 21.83 / 0.213 & 21.32 / 0.185 & 18.81 / 0.178 & 18.40 / 0.196 & 21.45 / 0.199 \\
% \hline
Ours w/ $\L_{sf}$ & 33 min & 22.36 / 0.121 & 28.99 / 0.062 & 25.07 / 0.093 & \textbf{23.91} / \textbf{0.094} & {22.36} / {0.121} & \textbf{25.31} / \textbf{0.072} & \textbf{22.76} / \textbf{0.070} & 24.55 / {0.086} \\
Ours w/o $\L_{sf}$ & 15 min & \textbf{23.45} / \textbf{0.100} & \textbf{29.98} / \textbf{0.045} & \textbf{25.22} / \textbf{0.090} & 23.24 / {0.096} & \textbf{23.75} / \textbf{0.079} & 24.15 / 0.081 & 22.19 / {0.074} & \textbf{24.57} / \textbf{0.081} \\ 
\hline
\end{tabular}
}
\label{tbl:supp_nvidia_scene_flow}
\end{table*}
